Hypervelocity Stars. I. The Spectroscopic Survey

We discuss our targeted search for hypervelocity stars (HVSs), stars traveling with velocities so extreme that dynamical ejection from a massive black hole is their only suggested origin. Our survey, now half complete, has successfully identified a total of four probable HVSs plus a number of other unusual objects. Here we report the most recently discovered two HVSs: SDSS J110557.45+093439.5 and possibly SDSS J113312.12+010824, traveling with Galactic rest-frame velocities at least +508+-12 and +418+-10 km/s, respectively. The other late B-type objects in our survey are consistent with a population of post main-sequence stars or blue stragglers in the Galactic halo, with mean metallicity [Fe/H]=-1.3 and velocity dispersion 108+-5 km/s. Interestingly, the velocity distribution shows a tail of objects with large positive velocities that may be a mix of low-velocity HVSs and high-velocity runaway stars. Our survey also includes a number of DA white dwarfs with unusually red colors, possibly extremely low mass objects. Two of our objects are B supergiants in the Leo A dwarf, providing the first spectroscopic evidence for star formation in this dwarf galaxy within the last ~30 Myr.

==> tab2.tex <==
 0:02:33.82 &  -9:57:06.8 & $18.578\pm0.021$ & $0.753\pm0.040$ & $-0.328\pm0.040$ & $ -88\pm10$ & $ 0.0\pm0.9$ \\
 0:05:28.14 & -11:00:10.1 & $19.271\pm0.042$ & $1.007\pm0.081$ & $-0.275\pm0.047$ & $-123\pm12$ & $-1.8\pm1.0$ \\
 0:07:52.01 &  -9:19:54.3 & $17.440\pm0.017$ & $1.016\pm0.036$ & $-0.276\pm0.039$ & $-119\pm11$ & $-1.6\pm0.6$ \\
 0:12:26.89 & -10:47:54.6 & $19.042\pm0.025$ & $1.006\pm0.064$ & $-0.321\pm0.038$ & $-132\pm11$ & $-0.2\pm1.0$ \\
 0:36:40.57 & -11:11:25.0 & $17.527\pm0.018$ & $0.778\pm0.028$ & $-0.304\pm0.031$ & $  27\pm10$ & $-1.8\pm0.4$ \\
 0:39:49.43 &   0:53:18.0 & $18.337\pm0.044$ & $1.133\pm0.059$ & $-0.294\pm0.048$ & $-130\pm10$ & $-1.3\pm0.9$ \\
 0:40:41.50 &  -9:01:34.0 & $17.424\pm0.032$ & $1.182\pm0.041$ & $-0.280\pm0.037$ & $-114\pm10$ & $-2.1\pm0.7$ \\
 0:52:02.29 &   1:08:40.8 & $18.041\pm0.015$ & $0.510\pm0.033$ & $-0.351\pm0.022$ & $-169\pm10$ & $ 0.0\pm0.5$ \\
 0:58:21.97 &  -8:51:29.3 & $18.819\pm0.035$ & $0.643\pm0.052$ & $-0.272\pm0.055$ & $-135\pm10$ & $-3.0\pm2.2$ \\
 1:12:35.80 &   0:48:18.7 & $17.593\pm0.024$ & $0.602\pm0.031$ & $-0.351\pm0.027$ & $ -62\pm10$ & $ 0.0\pm0.7$ \\
 1:14:02.57 &  14:04:40.9 & $18.560\pm0.022$ & $0.872\pm0.056$ & $-0.349\pm0.034$ & $-151\pm10$ & $-3.0\pm0.5$ \\
 1:24:02.39 &  -9:35:37.0 & $19.064\pm0.034$ & $1.061\pm0.066$ & $-0.281\pm0.039$ & $ -53\pm11$ & $-1.7\pm1.1$ \\
 1:26:51.70 &   0:47:21.7 & $19.829\pm0.021$ & $1.053\pm0.079$ & $-0.283\pm0.036$ & $-130\pm12$ & $-1.9\pm1.1$ \\
 1:36:40.69 & -10:29:44.5 & $17.909\pm0.057$ & $0.595\pm0.061$ & $-0.385\pm0.061$ & $-108\pm10$ & $-3.0\pm3.0$ \\
 1:43:18.95 & -10:31:36.6 & $19.894\pm0.054$ & $1.206\pm0.127$ & $-0.276\pm0.067$ & $-104\pm24$ & $-1.7\pm0.5$ \\
 1:45:08.38 &  -0:21:28.3 & $19.323\pm0.023$ & $0.398\pm0.042$ & $-0.354\pm0.029$ & $-157\pm10$ & $ 0.0\pm0.5$ \\
 1:49:06.96 &   0:57:47.3 & $19.357\pm0.024$ & $0.856\pm0.060$ & $-0.344\pm0.033$ & $-122\pm11$ & $ 0.0\pm0.5$ \\
 2:11:44.06 &  12:18:52.4 & $18.698\pm0.018$ & $0.743\pm0.038$ & $-0.290\pm0.034$ & $-198\pm10$ & $-0.7\pm1.0$ \\
 2:14:20.33 &  -8:19:57.7 & $17.387\pm0.018$ & $0.900\pm0.024$ & $-0.292\pm0.023$ & $ 225\pm10$ & $-1.2\pm0.9$ \\
 2:19:18.63 &  -8:57:57.7 & $18.759\pm0.024$ & $0.394\pm0.036$ & $-0.352\pm0.029$ & $-125\pm10$ & $ 0.0\pm0.6$ \\
 2:32:02.12 &  -0:45:37.6 & $19.074\pm0.023$ & $0.687\pm0.049$ & $-0.329\pm0.034$ & $-140\pm10$ & $ 0.0\pm1.3$ \\
 2:40:56.24 &  -0:31:22.4 & $19.807\pm0.032$ & $0.680\pm0.090$ & $-0.390\pm0.042$ & $ -11\pm11$ & $-3.0\pm3.0$ \\
 2:41:04.30 &   0:23:11.5 & $18.979\pm0.028$ & $1.072\pm0.062$ & $-0.325\pm0.032$ & $-138\pm10$ & $ 0.0\pm0.6$ \\
 3:02:04.20 &   0:32:14.9 & $18.039\pm0.023$ & $0.716\pm0.033$ & $-0.321\pm0.031$ & $ -58\pm10$ & $-0.0\pm1.6$ \\
 3:07:45.87 &  -7:25:28.9 & $18.385\pm0.029$ & $1.004\pm0.053$ & $-0.282\pm0.033$ & $-117\pm11$ & $-3.0\pm1.2$ \\
 3:20:54.69 &  -6:06:16.0 & $17.400\pm0.021$ & $0.707\pm0.033$ & $-0.318\pm0.025$ & $ 309\pm10$ & $-3.0\pm0.8$ \\
 7:35:58.72 &  40:24:27.9 & $18.422\pm0.014$ & $0.423\pm0.028$ & $-0.322\pm0.023$ & $  83\pm12$ & $-0.3\pm0.7$ \\
 7:41:21.83 &  32:48:17.3 & $18.687\pm0.016$ & $0.916\pm0.038$ & $-0.329\pm0.022$ & $  28\pm11$ & $ 0.0\pm0.5$ \\
 7:44:55.57 &  16:26:49.8 & $17.165\pm0.011$ & $0.432\pm0.021$ & $-0.346\pm0.014$ & $ 140\pm10$ & $ 0.0\pm0.5$ \\
 7:49:50.24 &  24:38:41.2 & $18.625\pm0.147$ & $0.745\pm0.151$ & $-0.342\pm0.148$ & $ 356\pm10$ & $ 0.0\pm0.5$ \\
 7:50:11.67 &  32:33:41.8 & $17.288\pm0.016$ & $0.483\pm0.023$ & $-0.320\pm0.019$ & $ -77\pm10$ & $-0.5\pm0.3$ \\
 7:56:37.60 &  16:34:34.2 & $17.723\pm0.019$ & $0.801\pm0.027$ & $-0.291\pm0.022$ & $ 135\pm12$ & $-0.8\pm0.4$ \\
 8:01:13.32 &  31:38:09.2 & $18.459\pm0.016$ & $1.020\pm0.038$ & $-0.274\pm0.023$ & $ -64\pm10$ & $-1.8\pm0.3$ \\
 8:08:11.98 &  27:35:37.8 & $18.422\pm0.017$ & $1.097\pm0.043$ & $-0.279\pm0.025$ & $ 176\pm11$ & $-1.4\pm0.5$ \\
 8:09:10.20 &  20:57:36.5 & $17.656\pm0.019$ & $0.327\pm0.028$ & $-0.372\pm0.023$ & $ 195\pm10$ & $ 0.0\pm0.5$ \\
 8:13:34.85 &   3:37:05.2 & $18.799\pm0.012$ & $0.730\pm0.034$ & $-0.285\pm0.017$ & $ 165\pm11$ & $-1.4\pm0.6$ \\
 8:16:10.59 &  25:04:06.0 & $19.429\pm0.023$ & $1.161\pm0.081$ & $-0.286\pm0.033$ & $ 230\pm10$ & $-1.9\pm1.2$ \\
 8:18:28.07 &  57:09:22.1 & $17.554\pm0.020$ & $0.791\pm0.030$ & $-0.313\pm0.024$ & $ 224\pm10$ & $-2.8\pm1.3$ \\
 8:21:04.19 &  22:18:43.5 & $17.573\pm0.014$ & $0.631\pm0.028$ & $-0.328\pm0.023$ & $ 104\pm10$ & $ 0.0\pm0.6$ \\
 8:21:11.56 &   2:00:56.8 & $17.135\pm0.014$ & $0.869\pm0.025$ & $-0.326\pm0.016$ & $ 258\pm10$ & $-2.9\pm2.0$ \\
 8:23:00.23 &  56:18:21.4 & $17.776\pm0.018$ & $0.902\pm0.029$ & $-0.316\pm0.025$ & $-150\pm11$ & $-0.2\pm0.7$ \\
 8:31:11.14 &  22:39:25.6 & $17.490\pm0.020$ & $0.670\pm0.032$ & $-0.335\pm0.023$ & $ -59\pm10$ & $ 0.0\pm0.5$ \\
 8:31:24.19 &   3:53:51.3 & $17.982\pm0.017$ & $0.456\pm0.026$ & $-0.311\pm0.028$ & $ -57\pm11$ & $-3.0\pm0.5$ \\
 8:32:11.86 &  40:44:59.4 & $17.973\pm0.016$ & $1.060\pm0.035$ & $-0.278\pm0.024$ & $  64\pm10$ & $-1.1\pm0.6$ \\
 8:35:03.10 &  21:43:39.9 & $17.342\pm0.015$ & $0.598\pm0.021$ & $-0.380\pm0.020$ & $ 191\pm10$ & $-3.0\pm3.0$ \\
 8:37:08.16 &  26:42:01.4 & $17.821\pm0.014$ & $1.116\pm0.031$ & $-0.304\pm0.021$ & $   5\pm11$ & $-1.4\pm0.5$ \\
 8:38:22.94 &   0:47:23.1 & $18.055\pm0.015$ & $0.946\pm0.034$ & $-0.331\pm0.021$ & $ 107\pm10$ & $ 0.0\pm0.6$ \\
 8:38:38.27 &  27:13:28.3 & $18.651\pm0.021$ & $1.046\pm0.043$ & $-0.279\pm0.026$ & $ -20\pm13$ & $ 0.0\pm0.5$ \\
 8:39:30.26 &  37:40:25.8 & $17.615\pm0.027$ & $0.884\pm0.047$ & $-0.287\pm0.035$ & $  37\pm10$ & $-0.2\pm0.9$ \\
 8:40:54.62 &  50:36:55.2 & $18.530\pm0.041$ & $0.669\pm0.057$ & $-0.381\pm0.045$ & $ 139\pm10$ & $-3.0\pm3.0$ \\
 8:43:50.65 &   4:59:33.5 & $17.790\pm0.012$ & $0.749\pm0.023$ & $-0.305\pm0.018$ & $ 265\pm10$ & $-1.2\pm0.8$ \\
 8:44:13.77 &   2:32:29.3 & $17.803\pm0.011$ & $0.615\pm0.032$ & $-0.294\pm0.017$ & $ 279\pm10$ & $-2.0\pm0.6$ \\
 8:44:54.11 &  37:20:10.6 & $18.296\pm0.020$ & $1.066\pm0.033$ & $-0.304\pm0.026$ & $ -95\pm10$ & $-1.4\pm0.9$ \\
 8:45:13.31 &  21:49:56.3 & $18.915\pm0.022$ & $0.935\pm0.050$ & $-0.303\pm0.030$ & $  31\pm10$ & $-1.2\pm0.4$ \\
 8:46:45.52 &  40:34:00.4 & $17.896\pm0.019$ & $1.050\pm0.044$ & $-0.306\pm0.024$ & $  -6\pm10$ & $-2.0\pm0.9$ \\
 8:50:22.46 &  47:13:19.4 & $17.138\pm0.020$ & $0.762\pm0.030$ & $-0.325\pm0.022$ & $-158\pm10$ & $-0.2\pm1.6$ \\
 8:50:35.53 &  54:53:13.3 & $17.284\pm0.020$ & $0.584\pm0.034$ & $-0.325\pm0.026$ & $-236\pm10$ & $-3.0\pm0.5$ \\
 8:51:19.70 &  40:31:37.4 & $17.926\pm0.021$ & $1.106\pm0.035$ & $-0.285\pm0.027$ & $ -84\pm11$ & $-1.3\pm0.9$ \\
 8:54:40.80 &   8:54:06.2 & $18.850\pm0.021$ & $0.986\pm0.050$ & $-0.277\pm0.028$ & $ 299\pm11$ & $-2.9\pm1.0$ \\
 9:01:38.58 &   0:33:04.2 & $17.539\pm0.012$ & $0.830\pm0.021$ & $-0.283\pm0.017$ & $ 340\pm10$ & $-3.0\pm0.5$ \\
 9:02:23.30 &  51:07:13.3 & $18.736\pm0.021$ & $1.023\pm0.056$ & $-0.304\pm0.028$ & $ 116\pm12$ & $-2.0\pm1.2$ \\
 9:05:59.15 &   5:54:42.1 & $17.995\pm0.018$ & $0.456\pm0.032$ & $-0.368\pm0.024$ & $ 319\pm10$ & $-3.0\pm0.5$ \\
 9:06:27.10 &   6:02:59.6 & $17.825\pm0.020$ & $0.799\pm0.031$ & $-0.292\pm0.024$ & $ 214\pm11$ & $-2.1\pm0.8$ \\
 9:07:10.08 &  36:59:57.5 & $18.159\pm0.021$ & $0.730\pm0.040$ & $-0.300\pm0.026$ & $ 301\pm10$ & $-1.4\pm0.5$ \\
 9:07:14.74 &   4:02:09.8 & $17.515\pm0.017$ & $0.379\pm0.025$ & $-0.358\pm0.021$ & $  14\pm10$ & $ 0.0\pm0.5$ \\
 9:10:31.31 &  37:45:15.6 & $17.317\pm0.021$ & $0.971\pm0.030$ & $-0.330\pm0.028$ & $  28\pm10$ & $ 0.0\pm0.5$ \\
 9:13:01.01 &  30:51:19.8 & $18.397\pm0.016$ & $0.367\pm0.028$ & $-0.361\pm0.023$ & $ 608\pm11$ & $ 0.0\pm2.0$ \\
 9:15:53.67 &  38:42:00.2 & $17.694\pm0.014$ & $0.841\pm0.025$ & $-0.360\pm0.027$ & $  29\pm10$ & $ 0.0\pm0.5$ \\
 9:17:59.48 &  67:22:38.3 & $17.932\pm0.021$ & $0.552\pm0.036$ & $-0.299\pm0.030$ & $ 548\pm11$ & $-2.8\pm1.8$ \\
 9:18:28.23 &   9:01:40.2 & $17.197\pm0.014$ & $0.641\pm0.024$ & $-0.333\pm0.019$ & $ 209\pm11$ & $-0.5\pm2.3$ \\
 9:27:02.63 &  46:28:57.3 & $19.527\pm0.029$ & $0.763\pm0.070$ & $-0.290\pm0.036$ & $ 113\pm10$ & $-1.0\pm1.2$ \\
 9:28:06.43 &  37:45:47.4 & $17.417\pm0.020$ & $1.107\pm0.028$ & $-0.327\pm0.034$ & $  67\pm11$ & $ 0.0\pm0.5$ \\
 9:44:46.92 &  47:07:10.7 & $17.811\pm0.021$ & $0.875\pm0.047$ & $-0.343\pm0.030$ & $  20\pm11$ & $ 0.0\pm0.5$ \\
 9:47:41.35 &  33:51:47.6 & $19.376\pm0.022$ & $0.624\pm0.047$ & $-0.331\pm0.030$ & $ 160\pm10$ & $ 0.0\pm0.5$ \\
 9:48:39.69 &  42:39:58.5 & $17.160\pm0.016$ & $0.942\pm0.031$ & $-0.314\pm0.018$ & $ -35\pm10$ & $ 0.0\pm0.6$ \\
 9:48:48.63 &  39:15:06.4 & $18.585\pm0.041$ & $1.117\pm0.057$ & $-0.318\pm0.049$ & $  -4\pm11$ & $-0.3\pm1.1$ \\
 9:49:52.40 &   7:55:12.1 & $18.386\pm0.029$ & $0.420\pm0.038$ & $-0.363\pm0.035$ & $ 105\pm11$ & $ 0.0\pm0.5$ \\
 9:51:25.45 &  60:00:18.2 & $17.735\pm0.024$ & $0.893\pm0.032$ & $-0.280\pm0.028$ & $ 112\pm12$ & $-1.7\pm0.6$ \\
 9:56:07.66 &  34:38:32.0 & $18.256\pm0.015$ & $0.633\pm0.034$ & $-0.314\pm0.023$ & $ 110\pm10$ & $-0.1\pm0.9$ \\
 9:56:33.32 &  55:33:06.6 & $19.346\pm0.033$ & $0.766\pm0.061$ & $-0.281\pm0.045$ & $   7\pm10$ & $-1.6\pm0.9$ \\
 9:59:15.12 &  30:44:10.4 & $19.896\pm0.025$ & $0.761\pm0.079$ & $-0.279\pm0.041$ & $  25\pm10$ & $-1.1\pm0.6$ \\
 9:59:20.22 &  30:43:52.7 & $19.435\pm0.024$ & $0.458\pm0.050$ & $-0.375\pm0.038$ & $  37\pm10$ & $ 0.0\pm0.5$ \\
10:00:19.08 &  33:11:05.4 & $18.966\pm0.018$ & $1.095\pm0.056$ & $-0.276\pm0.025$ & $  76\pm10$ & $-1.2\pm1.0$ \\
10:00:51.57 &  55:10:47.7 & $17.680\pm0.020$ & $0.936\pm0.032$ & $-0.321\pm0.027$ & $ -25\pm10$ & $-0.3\pm0.6$ \\
10:01:08.72 &   0:39:11.5 & $18.046\pm0.015$ & $0.755\pm0.026$ & $-0.313\pm0.023$ & $ 247\pm10$ & $-1.1\pm0.8$ \\
10:01:27.28 &   8:44:14.5 & $17.337\pm0.026$ & $1.189\pm0.032$ & $-0.283\pm0.035$ & $ 116\pm10$ & $-1.9\pm1.2$ \\
10:03:23.77 &  49:00:19.4 & $19.176\pm0.029$ & $1.030\pm0.083$ & $-0.285\pm0.040$ & $ -46\pm10$ & $-1.6\pm1.0$ \\
10:05:28.13 &  41:33:55.3 & $17.627\pm0.032$ & $0.997\pm0.039$ & $-0.279\pm0.038$ & $  68\pm10$ & $-1.7\pm1.1$ \\
10:06:35.70 &  69:07:28.1 & $17.987\pm0.020$ & $0.523\pm0.031$ & $-0.378\pm0.030$ & $-305\pm11$ & $-3.0\pm3.0$ \\
10:07:15.17 &  35:43:38.8 & $18.960\pm0.022$ & $0.979\pm0.049$ & $-0.288\pm0.032$ & $ 121\pm10$ & $-1.6\pm1.1$ \\
10:09:09.03 &  57:23:29.9 & $18.655\pm0.019$ & $0.979\pm0.042$ & $-0.294\pm0.030$ & $-165\pm11$ & $-1.0\pm1.3$ \\
10:09:17.91 &   2:38:00.3 & $18.171\pm0.020$ & $1.117\pm0.034$ & $-0.292\pm0.026$ & $  85\pm12$ & $ 0.0\pm0.5$ \\
10:10:25.63 &   4:53:57.0 & $18.256\pm0.014$ & $0.326\pm0.024$ & $-0.368\pm0.022$ & $  86\pm11$ & $ 0.0\pm2.1$ \\
10:13:02.73 &  60:38:08.0 & $18.470\pm0.036$ & $1.047\pm0.048$ & $-0.280\pm0.046$ & $-183\pm10$ & $-1.3\pm0.4$ \\
10:18:07.15 &  34:24:00.4 & $17.490\pm0.018$ & $1.016\pm0.031$ & $-0.274\pm0.029$ & $  34\pm10$ & $-1.8\pm0.6$ \\
10:20:14.35 &  33:42:52.4 & $18.758\pm0.014$ & $0.775\pm0.038$ & $-0.326\pm0.022$ & $ 175\pm10$ & $-0.2\pm1.0$ \\
10:21:01.93 &  60:26:29.2 & $19.180\pm0.019$ & $0.941\pm0.051$ & $-0.308\pm0.044$ & $  34\pm11$ & $-1.4\pm0.8$ \\
10:22:38.64 &  32:11:49.1 & $17.316\pm0.019$ & $1.136\pm0.027$ & $-0.278\pm0.028$ & $  55\pm16$ & $-0.9\pm0.7$ \\
10:22:56.35 &  11:43:20.4 & $17.771\pm0.020$ & $0.908\pm0.028$ & $-0.310\pm0.028$ & $  70\pm11$ & $-0.9\pm1.0$ \\
10:24:17.12 &  47:06:44.8 & $17.678\pm0.027$ & $0.740\pm0.043$ & $-0.321\pm0.034$ & $  33\pm10$ & $ 0.0\pm1.0$ \\
10:25:13.93 &  42:57:18.1 & $17.337\pm0.018$ & $0.698\pm0.025$ & $-0.366\pm0.023$ & $ 164\pm12$ & $ 0.0\pm0.5$ \\
10:25:54.94 &   9:01:14.4 & $18.709\pm0.016$ & $0.993\pm0.040$ & $-0.358\pm0.031$ & $ 294\pm11$ & $ 0.0\pm0.5$ \\
10:28:52.56 &  49:43:30.3 & $18.543\pm0.021$ & $0.589\pm0.031$ & $-0.296\pm0.031$ & $ -14\pm10$ & $-1.9\pm1.1$ \\
10:31:13.31 &  53:55:36.3 & $18.628\pm0.034$ & $1.068\pm0.060$ & $-0.273\pm0.043$ & $-129\pm10$ & $-2.9\pm1.3$ \\
10:33:32.41 &  54:10:30.5 & $18.874\pm0.018$ & $0.597\pm0.038$ & $-0.350\pm0.026$ & $ 100\pm10$ & $ 0.0\pm0.5$ \\
10:34:50.41 &  10:52:27.7 & $18.262\pm0.017$ & $0.625\pm0.031$ & $-0.321\pm0.028$ & $ 225\pm10$ & $-3.0\pm0.6$ \\
10:34:52.70 &   6:17:33.2 & $17.286\pm0.025$ & $1.067\pm0.031$ & $-0.307\pm0.035$ & $ 166\pm10$ & $ 0.0\pm0.8$ \\
10:39:41.15 &   7:16:10.4 & $19.117\pm0.019$ & $0.755\pm0.040$ & $-0.335\pm0.025$ & $ -42\pm10$ & $ 0.0\pm0.5$ \\
10:43:30.50 &  32:47:16.9 & $18.532\pm0.018$ & $1.049\pm0.039$ & $-0.276\pm0.022$ & $ 155\pm12$ & $-2.8\pm0.7$ \\
10:43:49.41 &  31:44:05.3 & $18.463\pm0.022$ & $0.946\pm0.041$ & $-0.350\pm0.030$ & $ 248\pm11$ & $ 0.0\pm0.5$ \\
10:46:10.16 &   9:50:43.9 & $19.237\pm0.024$ & $0.810\pm0.048$ & $-0.325\pm0.037$ & $  23\pm10$ & $ 0.0\pm1.0$ \\
10:47:33.18 &  10:05:57.5 & $18.534\pm0.019$ & $0.786\pm0.036$ & $-0.333\pm0.028$ & $ 312\pm10$ & $-2.9\pm1.1$ \\
10:49:13.15 &  51:02:32.7 & $19.475\pm0.024$ & $0.447\pm0.045$ & $-0.342\pm0.035$ & $ -12\pm10$ & $ 0.0\pm1.1$ \\
10:52:01.05 &  44:20:02.0 & $17.416\pm0.049$ & $0.945\pm0.053$ & $-0.369\pm0.052$ & $ -46\pm10$ & $ 0.0\pm1.1$ \\
10:53:37.93 &  30:26:40.1 & $18.525\pm0.012$ & $0.399\pm0.031$ & $-0.358\pm0.019$ & $ -31\pm10$ & $ 0.0\pm0.5$ \\
10:54:34.97 &  12:50:24.3 & $17.428\pm0.031$ & $1.016\pm0.036$ & $-0.296\pm0.036$ & $ 120\pm10$ & $-1.8\pm0.8$ \\
11:00:39.20 &  55:26:34.1 & $18.313\pm0.018$ & $0.646\pm0.031$ & $-0.313\pm0.025$ & $-139\pm10$ & $-0.3\pm0.8$ \\
11:02:24.37 &   2:50:02.8 & $18.139\pm0.016$ & $1.015\pm0.031$ & $-0.292\pm0.030$ & $ 446\pm10$ & $-0.5\pm1.1$ \\
11:04:22.82 &  38:45:19.7 & $17.341\pm0.020$ & $0.453\pm0.028$ & $-0.367\pm0.026$ & $ -21\pm10$ & $ 0.0\pm0.5$ \\
11:05:36.08 &   5:07:11.5 & $19.065\pm0.026$ & $0.758\pm0.054$ & $-0.316\pm0.040$ & $ 313\pm11$ & $-3.0\pm0.6$ \\
11:05:57.45 &   9:34:39.5 & $19.060\pm0.020$ & $0.714\pm0.045$ & $-0.299\pm0.029$ & $ 606\pm12$ & $-3.0\pm1.6$ \\
11:06:40.30 &  37:59:18.4 & $19.168\pm0.015$ & $0.673\pm0.040$ & $-0.307\pm0.023$ & $-145\pm10$ & $-0.6\pm1.1$ \\
11:06:51.52 &  58:17:04.1 & $18.703\pm0.028$ & $0.871\pm0.050$ & $-0.308\pm0.034$ & $ -31\pm10$ & $-1.4\pm0.3$ \\
11:09:35.08 &  58:03:08.4 & $17.265\pm0.025$ & $1.163\pm0.043$ & $-0.282\pm0.030$ & $-149\pm10$ & $-1.1\pm0.8$ \\
11:09:41.96 &  14:04:30.9 & $17.322\pm0.025$ & $1.018\pm0.035$ & $-0.296\pm0.030$ & $ 155\pm10$ & $-2.3\pm1.3$ \\
11:11:39.16 &   6:18:04.3 & $19.256\pm0.023$ & $0.979\pm0.062$ & $-0.313\pm0.031$ & $ 167\pm11$ & $-3.0\pm0.6$ \\
11:14:16.95 &  63:13:03.9 & $17.518\pm0.020$ & $1.068\pm0.028$ & $-0.290\pm0.024$ & $-224\pm11$ & $-3.0\pm0.5$ \\
11:14:18.12 &  12:46:03.2 & $17.485\pm0.024$ & $1.123\pm0.033$ & $-0.304\pm0.027$ & $ 165\pm10$ & $-3.0\pm0.5$ \\
11:14:20.06 &  45:28:46.3 & $18.909\pm0.030$ & $1.167\pm0.057$ & $-0.293\pm0.037$ & $-114\pm11$ & $-1.0\pm1.1$ \\
11:20:43.06 &   4:15:56.3 & $18.746\pm0.028$ & $0.617\pm0.041$ & $-0.325\pm0.036$ & $ 249\pm11$ & $-0.0\pm1.4$ \\
11:20:58.97 &   4:20:12.4 & $17.857\pm0.023$ & $0.763\pm0.030$ & $-0.304\pm0.028$ & $ 278\pm10$ & $-3.0\pm0.5$ \\
11:24:38.17 &  61:13:47.7 & $17.856\pm0.018$ & $0.855\pm0.032$ & $-0.311\pm0.031$ & $-114\pm10$ & $-2.0\pm1.5$ \\
11:28:30.43 &  -1:21:33.0 & $18.288\pm0.021$ & $1.060\pm0.035$ & $-0.310\pm0.032$ & $ -59\pm10$ & $-1.6\pm0.9$ \\
11:31:55.15 &  12:51:06.8 & $18.185\pm0.102$ & $1.154\pm0.108$ & $-0.296\pm0.498$ & $ 291\pm10$ & $-1.6\pm0.4$ \\
11:33:12.12 &   1:08:24.9 & $17.749\pm0.019$ & $0.468\pm0.025$ & $-0.322\pm0.024$ & $ 531\pm10$ & $-0.0\pm1.7$ \\
11:37:15.32 &  56:22:04.3 & $17.740\pm0.032$ & $1.211\pm0.045$ & $-0.285\pm0.043$ & $ -89\pm13$ & $-1.0\pm1.1$ \\
11:37:53.83 &   7:17:52.8 & $18.201\pm0.029$ & $0.602\pm0.043$ & $-0.320\pm0.035$ & $ 196\pm10$ & $-3.0\pm0.5$ \\
11:37:57.16 &  -0:32:00.4 & $17.098\pm0.029$ & $0.858\pm0.036$ & $-0.312\pm0.035$ & $  72\pm10$ & $-1.8\pm0.7$ \\
11:38:32.81 &  40:23:25.4 & $17.863\pm0.018$ & $1.099\pm0.040$ & $-0.307\pm0.022$ & $-100\pm12$ & $-0.0\pm0.9$ \\
11:40:18.82 &  10:24:06.0 & $18.048\pm0.021$ & $1.032\pm0.030$ & $-0.271\pm0.026$ & $ 108\pm11$ & $-1.6\pm0.8$ \\
11:41:53.49 &   2:11:15.3 & $17.490\pm0.017$ & $1.116\pm0.029$ & $-0.304\pm0.022$ & $  60\pm11$ & $-0.4\pm0.4$ \\
11:43:08.15 &   1:38:57.2 & $17.282\pm0.020$ & $0.653\pm0.028$ & $-0.351\pm0.024$ & $ 313\pm10$ & $ 0.0\pm2.2$ \\
11:52:45.91 &  -2:11:16.2 & $18.215\pm0.020$ & $0.959\pm0.030$ & $-0.344\pm0.026$ & $ 419\pm11$ & $ 0.0\pm0.5$ \\
11:57:25.71 &  12:55:34.2 & $17.456\pm0.017$ & $1.170\pm0.033$ & $-0.291\pm0.035$ & $  80\pm11$ & $-1.4\pm0.6$ \\
12:17:55.47 &  37:29:38.8 & $18.122\pm0.021$ & $0.979\pm0.035$ & $-0.289\pm0.028$ & $ -15\pm11$ & $-1.1\pm0.8$ \\
12:20:08.00 &  38:57:53.8 & $17.580\pm0.026$ & $0.860\pm0.033$ & $-0.292\pm0.029$ & $-111\pm11$ & $-1.4\pm0.5$ \\
12:20:24.75 &  31:59:53.4 & $17.134\pm0.018$ & $0.988\pm0.030$ & $-0.293\pm0.022$ & $  28\pm10$ & $-1.6\pm0.5$ \\
12:22:56.65 &  39:12:14.6 & $18.534\pm0.015$ & $0.633\pm0.033$ & $-0.328\pm0.022$ & $-146\pm10$ & $-0.3\pm1.1$ \\
12:32:58.59 &  31:34:14.8 & $17.305\pm0.020$ & $0.910\pm0.035$ & $-0.292\pm0.024$ & $-143\pm10$ & $-3.0\pm0.5$ \\
12:56:10.99 &  40:36:11.6 & $17.367\pm0.029$ & $0.820\pm0.046$ & $-0.280\pm0.032$ & $-138\pm10$ & $-2.2\pm1.0$ \\
13:04:07.10 &  43:11:08.7 & $17.466\pm0.022$ & $0.511\pm0.038$ & $-0.338\pm0.029$ & $ 152\pm10$ & $ 0.0\pm2.0$ \\
13:07:53.64 &  30:35:52.1 & $18.340\pm0.019$ & $0.436\pm0.037$ & $-0.336\pm0.025$ & $ -33\pm10$ & $ 0.0\pm1.1$ \\
13:13:38.71 &  32:19:05.8 & $17.415\pm0.025$ & $1.098\pm0.033$ & $-0.272\pm0.031$ & $ -69\pm10$ & $-1.5\pm0.7$ \\
13:13:58.21 &  30:04:37.9 & $18.104\pm0.020$ & $0.480\pm0.062$ & $-0.338\pm0.026$ & $ -84\pm10$ & $ 0.0\pm1.1$ \\
13:21:55.16 &  31:28:58.6 & $18.983\pm0.019$ & $0.916\pm0.044$ & $-0.336\pm0.039$ & $-202\pm11$ & $-3.0\pm0.6$ \\
13:34:26.43 &  41:01:02.5 & $17.341\pm0.027$ & $0.597\pm0.037$ & $-0.349\pm0.035$ & $-234\pm10$ & $ 0.0\pm1.3$ \\
14:06:35.27 &  56:44:20.2 & $18.347\pm0.026$ & $0.711\pm0.036$ & $-0.310\pm0.032$ & $-163\pm10$ & $ 0.0\pm0.9$ \\
14:07:44.53 &  60:40:08.2 & $17.322\pm0.026$ & $1.032\pm0.035$ & $-0.295\pm0.029$ & $ -35\pm10$ & $-1.1\pm0.7$ \\
14:09:45.27 &  41:42:56.9 & $19.260\pm0.017$ & $1.037\pm0.055$ & $-0.278\pm0.025$ & $-123\pm11$ & $-3.0\pm0.5$ \\
14:27:37.92 &  50:00:55.1 & $19.380\pm0.018$ & $0.791\pm0.064$ & $-0.300\pm0.028$ & $-295\pm22$ & $-1.3\pm1.5$ \\
14:28:46.70 &  35:31:57.3 & $17.462\pm0.017$ & $0.522\pm0.036$ & $-0.336\pm0.023$ & $-165\pm10$ & $-2.6\pm0.3$ \\
14:31:15.16 &  63:11:30.1 & $17.470\pm0.017$ & $1.066\pm0.027$ & $-0.286\pm0.022$ & $ -38\pm10$ & $-1.1\pm0.7$ \\
14:31:57.10 &  35:28:00.0 & $18.991\pm0.026$ & $1.030\pm0.050$ & $-0.281\pm0.032$ & $-210\pm18$ & $-1.9\pm0.7$ \\
14:32:24.31 &  37:02:12.9 & $17.679\pm0.019$ & $1.041\pm0.030$ & $-0.308\pm0.026$ & $-205\pm11$ & $-3.0\pm0.5$ \\
14:33:47.48 &  50:17:18.1 & $17.647\pm0.038$ & $0.995\pm0.045$ & $-0.344\pm0.040$ & $-337\pm10$ & $-2.5\pm0.3$ \\
14:40:18.90 &  39:46:24.1 & $17.329\pm0.025$ & $0.988\pm0.033$ & $-0.271\pm0.030$ & $-250\pm10$ & $-0.6\pm0.5$ \\
14:43:04.91 &  44:53:05.1 & $17.304\pm0.021$ & $0.867\pm0.033$ & $-0.287\pm0.030$ & $-111\pm10$ & $-1.5\pm0.8$ \\
14:49:34.28 &  49:29:26.7 & $17.512\pm0.018$ & $0.586\pm0.026$ & $-0.337\pm0.022$ & $-168\pm10$ & $ 0.0\pm0.5$ \\
15:01:09.63 &  42:29:21.4 & $18.332\pm0.014$ & $1.059\pm0.030$ & $-0.278\pm0.021$ & $ -84\pm10$ & $-0.0\pm1.1$ \\
15:02:35.75 &  38:16:17.0 & $17.223\pm0.021$ & $0.626\pm0.044$ & $-0.294\pm0.026$ & $-342\pm10$ & $-1.9\pm0.5$ \\
15:23:01.89 &  40:20:56.8 & $19.493\pm0.029$ & $1.063\pm0.075$ & $-0.307\pm0.048$ & $-110\pm12$ & $ 0.0\pm0.7$ \\
15:24:01.54 &  50:51:12.6 & $17.584\pm0.028$ & $0.998\pm0.038$ & $-0.271\pm0.036$ & $ -75\pm16$ & $-1.8\pm0.5$ \\
15:28:12.09 &  52:46:40.5 & $19.252\pm0.021$ & $0.936\pm0.054$ & $-0.275\pm0.028$ & $-195\pm14$ & $-1.0\pm0.8$ \\
15:30:42.16 &  30:28:22.4 & $17.673\pm0.019$ & $1.058\pm0.036$ & $-0.283\pm0.024$ & $ -27\pm11$ & $-0.4\pm0.4$ \\
15:38:29.27 &  34:48:21.1 & $17.550\pm0.012$ & $0.672\pm0.026$ & $-0.284\pm0.018$ & $-118\pm10$ & $-0.6\pm0.7$ \\
15:41:38.99 &  34:06:50.5 & $18.547\pm0.013$ & $0.643\pm0.032$ & $-0.338\pm0.020$ & $ -96\pm10$ & $ 0.0\pm0.5$ \\
15:42:55.88 &  30:19:46.2 & $19.474\pm0.024$ & $1.078\pm0.058$ & $-0.272\pm0.032$ & $-205\pm14$ & $-1.4\pm0.5$ \\
15:44:50.02 &  43:17:21.2 & $17.801\pm0.016$ & $0.694\pm0.026$ & $-0.294\pm0.027$ & $ -58\pm10$ & $-0.9\pm0.5$ \\
15:46:15.99 &  34:38:21.1 & $18.745\pm0.018$ & $0.737\pm0.037$ & $-0.312\pm0.025$ & $   7\pm10$ & $ 0.0\pm0.5$ \\
15:49:16.62 &  36:30:23.9 & $18.258\pm0.016$ & $0.704\pm0.033$ & $-0.359\pm0.027$ & $-174\pm10$ & $ 0.0\pm0.5$ \\
15:52:35.89 &  41:47:45.4 & $18.261\pm0.023$ & $0.828\pm0.041$ & $-0.304\pm0.027$ & $ -34\pm10$ & $-0.7\pm0.9$ \\
16:03:47.08 &  26:02:54.4 & $17.276\pm0.014$ & $0.889\pm0.024$ & $-0.295\pm0.026$ & $-194\pm10$ & $-1.7\pm0.9$ \\
16:04:07.94 &  49:38:54.4 & $17.608\pm0.018$ & $0.807\pm0.035$ & $-0.329\pm0.023$ & $-277\pm16$ & $ 0.0\pm0.5$ \\
16:06:08.01 &  39:35:10.6 & $17.692\pm0.016$ & $0.864\pm0.026$ & $-0.297\pm0.023$ & $-315\pm10$ & $-0.1\pm1.4$ \\
16:07:54.77 &  31:39:44.1 & $17.541\pm0.014$ & $0.744\pm0.024$ & $-0.313\pm0.021$ & $-197\pm11$ & $-3.0\pm0.7$ \\
16:09:51.52 &  32:42:03.2 & $18.521\pm0.021$ & $1.030\pm0.043$ & $-0.303\pm0.028$ & $-145\pm10$ & $-0.5\pm0.5$ \\
16:12:30.96 &  34:10:46.7 & $17.523\pm0.025$ & $1.057\pm0.035$ & $-0.303\pm0.033$ & $-245\pm11$ & $-0.4\pm1.1$ \\
16:13:01.66 &  39:00:44.1 & $18.113\pm0.016$ & $1.136\pm0.032$ & $-0.275\pm0.022$ & $-204\pm11$ & $-1.1\pm0.8$ \\
16:19:06.60 &  42:41:18.1 & $17.894\pm0.017$ & $0.962\pm0.028$ & $-0.278\pm0.022$ & $-203\pm10$ & $-2.2\pm0.7$ \\
16:47:53.84 &  63:58:33.9 & $19.688\pm0.027$ & $0.520\pm0.059$ & $-0.362\pm0.040$ & $-259\pm11$ & $-3.0\pm0.5$ \\
16:59:11.34 &  62:09:51.7 & $18.523\pm0.017$ & $0.757\pm0.034$ & $-0.341\pm0.029$ & $ -30\pm10$ & $ 0.0\pm0.5$ \\
17:03:28.38 &  65:34:39.3 & $17.349\pm0.020$ & $0.838\pm0.028$ & $-0.281\pm0.026$ & $-350\pm11$ & $-3.0\pm0.6$ \\
17:11:34.54 &  59:58:31.4 & $18.319\pm0.023$ & $0.809\pm0.034$ & $-0.282\pm0.027$ & $-144\pm10$ & $-0.3\pm0.4$ \\
17:14:52.25 &  62:07:16.7 & $17.561\pm0.031$ & $0.805\pm0.039$ & $-0.362\pm0.034$ & $-180\pm10$ & $ 0.0\pm0.5$ \\
17:20:04.07 &  57:51:10.8 & $18.435\pm0.015$ & $1.060\pm0.039$ & $-0.280\pm0.019$ & $-276\pm10$ & $-1.6\pm0.8$ \\
22:03:34.63 &  -0:29:56.4 & $17.371\pm0.022$ & $0.843\pm0.028$ & $-0.278\pm0.027$ & $ -57\pm10$ & $-1.0\pm0.7$ \\
22:29:51.51 &   0:32:14.1 & $17.440\pm0.019$ & $0.801\pm0.027$ & $-0.271\pm0.024$ & $-166\pm10$ & $-1.5\pm0.7$ \\
22:34:36.89 &   0:22:24.7 & $17.611\pm0.016$ & $1.052\pm0.031$ & $-0.302\pm0.019$ & $-204\pm12$ & $ 0.0\pm0.5$ \\
22:41:05.19 &  14:18:10.2 & $18.635\pm0.016$ & $0.416\pm0.030$ & $-0.367\pm0.021$ & $-204\pm10$ & $-2.7\pm0.3$ \\
22:55:44.31 &  -8:14:25.7 & $17.499\pm0.016$ & $0.425\pm0.027$ & $-0.371\pm0.023$ & $ 107\pm10$ & $ 0.0\pm0.5$ \\
22:59:57.44 &  -9:38:21.8 & $17.203\pm0.019$ & $0.988\pm0.040$ & $-0.276\pm0.025$ & $-129\pm10$ & $-1.2\pm0.9$ \\
23:21:09.36 &  14:58:01.1 & $18.153\pm0.014$ & $0.460\pm0.025$ & $-0.361\pm0.022$ & $-144\pm10$ & $ 0.0\pm0.5$ \\


==> tab3.tex <==
 0:28:03.34 &  -0:12:13.4 & $18.414\pm0.019$ & $0.517\pm0.032$ & $-0.418\pm0.025$ & $  97\pm43$ \\
 1:00:44.69 &  -0:50:34.1 & $20.111\pm0.062$ & $0.577\pm0.097$ & $-0.300\pm0.068$ & $  73\pm47$ \\
 1:06:57.83 & -10:08:39.3 & $19.417\pm0.025$ & $0.525\pm0.072$ & $-0.366\pm0.035$ & $ -23\pm47$ \\
 1:11:30.67 &  14:10:49.7 & $19.984\pm0.040$ & $0.379\pm0.075$ & $-0.357\pm0.054$ & $ -12\pm29$ \\
 2:02:32.30 &  -8:49:18.3 & $19.218\pm0.088$ & $0.481\pm0.098$ & $-0.346\pm0.097$ & $  59\pm61$ \\
 3:12:40.49 &  -0:59:41.1 & $19.648\pm0.050$ & $0.283\pm0.069$ & $-0.411\pm0.170$ & $ 129\pm53$ \\
 7:37:34.88 &  21:50:17.3 & $19.369\pm0.016$ & $0.458\pm0.049$ & $-0.320\pm0.026$ & $  51\pm25$ \\
 7:45:08.15 &  18:26:30.0 & $19.420\pm0.016$ & $0.751\pm0.051$ & $-0.404\pm0.025$ & $  61\pm37$ \\
 7:56:37.74 &  20:37:30.7 & $18.830\pm0.013$ & $0.230\pm0.030$ & $-0.416\pm0.019$ & $ -44\pm42$ \\
 8:02:34.62 &  43:23:01.1 & $18.536\pm0.020$ & $0.432\pm0.034$ & $-0.347\pm0.025$ & $  62\pm35$ \\
 8:20:03.03 &  25:00:12.1 & $19.559\pm0.021$ & $0.450\pm0.051$ & $-0.382\pm0.040$ & $  20\pm41$ \\
 8:25:42.49 &   8:01:00.5 & $19.474\pm0.028$ & $0.451\pm0.050$ & $-0.365\pm0.037$ & $  77\pm40$ \\
 8:28:23.55 &  47:00:01.4 & $17.764\pm0.058$ & $0.423\pm0.065$ & $-0.322\pm0.112$ & $  97\pm40$ \\
 8:33:03.03 &  36:59:06.3 & $18.054\pm0.019$ & $0.948\pm0.080$ & $-0.283\pm0.029$ & $  19\pm50$ \\
 8:48:23.75 &   5:08:45.2 & $17.268\pm0.013$ & $0.272\pm0.021$ & $-0.376\pm0.023$ & $  -6\pm26$ \\
 8:51:41.58 &  42:51:17.7 & $18.366\pm0.027$ & $0.492\pm0.035$ & $-0.304\pm0.034$ & $  56\pm39$ \\
 8:56:52.65 &  23:33:41.8 & $18.494\pm0.015$ & $0.311\pm0.027$ & $-0.401\pm0.024$ & $  11\pm43$ \\
 8:58:59.83 &   5:07:57.2 & $19.188\pm0.025$ & $0.396\pm0.048$ & $-0.357\pm0.032$ & $  33\pm42$ \\
 9:17:09.55 &  46:38:21.8 & $18.747\pm0.019$ & $0.738\pm0.037$ & $-0.328\pm0.024$ & $ 165\pm12$ \\
 9:20:01.94 &   0:52:01.1 & $19.407\pm0.021$ & $0.440\pm0.042$ & $-0.373\pm0.030$ & $  93\pm43$ \\
 9:29:18.13 &  37:45:29.9 & $19.384\pm0.059$ & $0.470\pm0.070$ & $-0.377\pm0.066$ & $ -79\pm26$ \\
 9:39:55.29 &   5:49:34.6 & $18.379\pm0.029$ & $0.539\pm0.038$ & $-0.345\pm0.034$ & $  10\pm34$ \\
 9:50:30.48 &  38:57:13.2 & $18.415\pm0.022$ & $0.321\pm0.034$ & $-0.400\pm0.036$ & $  72\pm35$ \\
 9:56:41.27 &  68:57:27.5 & $18.358\pm0.133$ & $0.550\pm0.140$ & $-0.372\pm0.629$ & $ -23\pm33$ \\
 9:57:17.31 &  55:28:39.2 & $18.712\pm0.051$ & $0.352\pm0.056$ & $-0.388\pm0.056$ & $  43\pm40$ \\
10:03:54.41 &   6:38:50.6 & $19.222\pm0.019$ & $0.417\pm0.042$ & $-0.336\pm0.033$ & $  44\pm32$ \\
10:06:18.54 &  60:55:00.7 & $18.203\pm0.026$ & $0.550\pm0.034$ & $-0.283\pm0.035$ & $  60\pm35$ \\
10:09:29.84 &  41:12:05.2 & $19.474\pm0.044$ & $0.404\pm0.063$ & $-0.348\pm0.049$ & $ -59\pm39$ \\
10:15:19.62 &  59:54:30.5 & $17.962\pm0.023$ & $0.544\pm0.034$ & $-0.309\pm0.032$ & $  31\pm39$ \\
10:15:57.01 &  51:04:28.4 & $18.747\pm0.019$ & $0.574\pm0.035$ & $-0.347\pm0.031$ & $   1\pm28$ \\
10:16:47.50 &  37:58:35.2 & $17.333\pm0.041$ & $0.375\pm0.048$ & $-0.402\pm0.042$ & $ -41\pm46$ \\
10:46:50.53 &  51:00:28.6 & $17.924\pm0.027$ & $0.419\pm0.031$ & $-0.402\pm0.032$ & $  28\pm35$ \\
10:53:53.89 &  52:00:31.0 & $18.928\pm0.023$ & $0.395\pm0.049$ & $-0.358\pm0.045$ & $ -53\pm18$ \\
10:58:50.47 &  43:27:10.9 & $18.979\pm0.030$ & $0.450\pm0.044$ & $-0.372\pm0.037$ & $ -54\pm24$ \\
11:02:00.07 &  -0:40:55.9 & $19.243\pm0.027$ & $0.333\pm0.041$ & $-0.363\pm0.035$ & $   0\pm35$ \\
11:11:33.37 &  13:46:39.8 & $19.437\pm0.018$ & $0.694\pm0.224$ & $-0.328\pm0.038$ & $   0\pm70$ \\
11:19:08.64 &   3:38:18.6 & $19.061\pm0.039$ & $0.403\pm0.063$ & $-0.338\pm0.045$ & $   9\pm41$ \\
11:38:07.13 &  14:32:57.4 & $17.764\pm0.032$ & $0.597\pm0.036$ & $-0.284\pm0.037$ & $  54\pm22$ \\
11:43:44.96 &   5:22:14.8 & $17.445\pm0.028$ & $0.441\pm0.038$ & $-0.358\pm0.054$ & $ -59\pm34$ \\
14:58:59.60 &  43:11:13.3 & $19.265\pm0.025$ & $0.539\pm0.042$ & $-0.323\pm0.031$ & $ -68\pm64$ \\
15:10:27.67 &  41:25:20.1 & $19.080\pm0.032$ & $0.484\pm0.046$ & $-0.352\pm0.050$ & $  65\pm63$ \\
15:18:52.49 &  53:01:21.8 & $19.103\pm0.013$ & $0.866\pm0.053$ & $-0.367\pm0.025$ & $ -89\pm16$ \\
15:29:05.82 &  33:05:20.4 & $18.392\pm0.020$ & $0.575\pm0.037$ & $-0.330\pm0.027$ & $ -65\pm44$ \\
15:57:08.48 &  28:23:36.0 & $17.648\pm0.029$ & $0.532\pm0.036$ & $-0.365\pm0.033$ & $ 145\pm29$ \\

